Efficient 3D Semantic Segmentation with Superpoint Transformer

We introduce a novel superpoint-based transformer architecture for efficient semantic segmentation of large-scale 3D scenes. Our method incorporates a fast algorithm to partition point clouds into a hierarchical superpoint structure, which makes our preprocessing 7 times faster than existing superpoint-based approaches. Additionally, we leverage a self-attention mechanism to capture the relationships between superpoints at multiple scales, leading to state-of-the-art performance on three challenging benchmark datasets: S3DIS (76.0% mIoU 6-fold validation), KITTI-360 (63.5% on Val), and DALES (79.6%). With only 212k parameters, our approach is up to 200 times more compact than other state-of-the-art models while maintaining similar performance. Furthermore, our model can be trained on a single GPU in 3 hours for a fold of the S3DIS dataset, which is 7x to 70x fewer GPU-hours than the best-performing methods. Our code and models are accessible at github.com/drprojects/superpoint_transformer.

==> figures/visualizer_in_title.tex <==
\begin{center}
\centering

\begin{tabular}{@{}ccc@{}}
\includegraphics[width=.3\linewidth]{images/interactive_tool/position.jpg}
&
\includegraphics[width=.3\linewidth]{images/interactive_tool/labels.jpg}
&
\includegraphics[width=.3\linewidth]{images/interactive_tool/features.jpg}
\\
a) Position & b) Ground Truth  & c) \textcolor{red}{Linearity}, \textcolor{green}{Planarity} \& \textcolor{blue}{Verticality}
\\
\includegraphics[width=.3\linewidth]{images/interactive_tool/rgb.jpg}
&
\includegraphics[width=.3\linewidth]{images/interactive_tool/predictions_with_errors.jpg}
&
\includegraphics[width=.35\linewidth]{images/interactive_tool/level_2.jpg}
\\
d) RGB & e) Predictions \& \textcolor{red}{Errors} & f) Level-2 
\end{tabular}
\captionsetup{type=figure}
\captionof{figure}{{\bf Interactive Visualization.} Our interactive viewing tool allows for the manipulation and visualization of sample point clouds colorized according to their position (a), semantic labels (b), selected geometric features (c), radiometry (d), and to visualize our network's prediction (e) and partitions (f).}
 \label{fig:visu}
\end{center}
